Fair Attribute Classification through Latent Space De-biasing

Fairness in visual recognition is becoming a prominent and critical topic of discussion as recognition systems are deployed at scale in the real world. Models trained from data in which target labels are correlated with protected attributes (e.g., gender, race) are known to learn and exploit those correlations. In this work, we introduce a method for training accurate target classifiers while mitigating biases that stem from these correlations. We use GANs to generate realistic-looking images, and perturb these images in the underlying latent space to generate training data that is balanced for each protected attribute. We augment the original dataset with this perturbed generated data, and empirically demonstrate that target classifiers trained on the augmented dataset exhibit a number of both quantitative and qualitative benefits. We conduct a thorough evaluation across multiple target labels and protected attributes in the CelebA dataset, and provide an in-depth analysis and comparison to existing literature in the space.

==> GAN debiasing CVPR/baseline_comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|c|c c || c c|}
% \cline{2-4}
% & \multicolumn{1}{|c}{Baseline} & Ours &  {\sc model\_inv} \\ \hline 
% \multicolumn{4}{|l|}{AP $\uparrow$}\\ \hline
\hline
\multirow{2}{*}{Attr. type}& \multicolumn{2}{c||}{AP $\uparrow$} & \multicolumn{2}{c|}{DEO $\downarrow$} \\
\cline{2-5} 
 & Baseline & Ours & Baseline & Ours \\ \hline
\multicolumn{1}{|c|}{Incons.} & \textbf{66.3 $\pm$ 1.8} & 65.2 $\pm$ 1.9 & 21.5 $\pm$ 4.4 & \textbf{16.5 $\pm$ 4.2} \\
\multicolumn{1}{|c|}{G-dep} & \textbf{78.6 $\pm$ 1.4} & 77.8 $\pm$ 1.4 & 25.7 $\pm$ 3.5 & \textbf{23.4 $\pm$ 3.6} \\
\multicolumn{1}{|c|}{G-indep.} & \textbf{83.9 $\pm$ 1.5} & 83.0 $\pm$ 1.6 & 16.7 $\pm$ 5.0 & \textbf{13.9 $\pm$ 5.2} \\
\hline 
\multirow{2}{*}{Attr. type}& \multicolumn{2}{c||}{BA $\downarrow$} & \multicolumn{2}{c|}{KL $\downarrow$} \\
\cline{2-5} 
& Baseline & Ours & Baseline & Ours \\ \hline
\multicolumn{1}{|c|}{Incons.} & 2.1 $\pm$ 0.6 & \textbf{0.5 $\pm$ 0.6} & 1.7 $\pm$ 0.3 & \textbf{1.3 $\pm$ 0.4} \\
\multicolumn{1}{|c|}{G-dep} &  2.3 $\pm$ 0.5 & \textbf{1.6 $\pm$ 0.5} & 1.3 $\pm$ 0.2 & \textbf{1.2 $\pm$ 0.2}\\
\multicolumn{1}{|c|}{G-indep.} & 0.3 $\pm$ 0.6 & \textbf{0.0 $\pm$ 0.5} &  1.1 $\pm$ 0.5 & \textbf{0.9 $\pm$ 0.6}\\
\hline 
\end{tabular}

% \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Our Model \\ (FAIR GAN)\end{tabular}}
\begin{comment}
% Averaged table
\begin{tabular}{|c|c c c|}
% \cline{2-4}
% & \multicolumn{1}{|c}{Baseline} & Ours &  {\sc model\_inv} \\ \hline 
% \multicolumn{4}{|l|}{AP $\uparrow$}\\ \hline
\hline AP $\uparrow$ & Baseline & Ours & {\sc model\_inv} \\ \hline
\multicolumn{1}{|c|}{Inconsistently labeled} & \textbf{66.3 $\pm$ 1.8} & 65.2 $\pm$ 1.9 & 65.2 $\pm$ 1.6 \\
\multicolumn{1}{|c|}{Gender-dependent} & \textbf{78.6 $\pm$ 1.4} & 77.8 $\pm$ 1.4 & 77.4 $\pm$ 1.2 \\
\multicolumn{1}{|c|}{Gender-independent} & \textbf{83.9 $\pm$ 1.5} & 83.0 $\pm$ 1.6 & 83.0 $\pm$ 1.8\\
% \hline \multicolumn{4}{|l|}{DEO $\downarrow$}\\ \hline
\hline DEO $\downarrow$ & Baseline & Ours & {\sc model\_inv} \\ \hline
\multicolumn{1}{|c|}{Inconsistently labeled} & 19.6 $\pm$ 4.3 & \textbf{14.5 $\pm$ 4.1} & 16.3 $\pm$ 3.8  \\
\multicolumn{1}{|c|}{Gender-dependent} & 23.0 $\pm$ 3.6 & 21.8 $\pm$ 3.8 & \textbf{19.1 $\pm$ 3.3} \\
\multicolumn{1}{|c|}{Gender-independent} & 16.6 $\pm$ 5.1 & 13.6 $\pm$ 5.1 & \textbf{12.7 $\pm$ 4.2} \\
% \hline \multicolumn{4}{|l|}{DNAP $\downarrow$}\\ \hline
% \hline \multicolumn{4}{|l|}{Bias Amplification $\downarrow$}\\ \hline
\hline BA $\downarrow$ & Baseline & Ours & {\sc model\_inv} \\ \hline
\multicolumn{1}{|c|}{Inconsistently labeled} & 2.9 $\pm$ 0.6 & 1.6 $\pm$ 0.6 & \textbf{0.7 $\pm$ 0.6}  \\
\multicolumn{1}{|c|}{Gender-dependent} & 3.1 $\pm$ 0.5 & 3.0 $\pm$ 0.5 & \textbf{2.5 $\pm$ 0.6} \\
\multicolumn{1}{|c|}{Gender-independent} & 0.7 $\pm$ 0.5 & \textbf{0.4 $\pm$ 0.5} & 0.5 $\pm$ 0.4 \\
% \hline DNAP $\downarrow$ & Baseline & Ours & {\sc model\_inv} \\ \hline
% \multicolumn{1}{|c|}{Inconsistently labeled} & 10.2 $\pm$ 3.7 & \textbf{9.9 $\pm$ 3.6} & \textbf{9.9 $\pm$ 3.0}  \\
% \multicolumn{1}{|c|}{Gender-dependent} &\textbf{7.6 $\pm$ 2.3} & 7.8 $\pm$ 2.7 & 8.3 $\pm$ 2.5 \\
% \multicolumn{1}{|c|}{Gender-independent} & 3.6 $\pm$ 3.0 & 3.6 $\pm$ 3.2 & \textbf{3.5 $\pm$ 2.6} \\
\hline KL $\downarrow$ & Baseline & Ours & {\sc model\_inv} \\ \hline
\multicolumn{1}{|c|}{Inconsistently labeled} & 1.70 $\pm$ 0.31 & \textbf{1.33 $\pm$ 0.25} & 1.45 $\pm$ 0.29 \\
\multicolumn{1}{|c|}{Gender-dependent} & 1.30 $\pm$ 0.15 & \textbf{1.18 $\pm$ 0.15} & \textbf{1.18 $\pm$ 0.14} \\
\multicolumn{1}{|c|}{Gender-independent} & 1.10 $\pm$ 0.45 & 0.93 $\pm$ 0.36 & \textbf{0.87 $\pm$ 0.36} \\
\hline
\end{tabular}
\end{comment}

\begin{comment}
\begin{tabular}{|c|ccc|ccc|}
\hline
 & \multicolumn{3}{c}{AP $\uparrow$} & \multicolumn{3}{|c|}{DEO $\downarrow$} \\ \hline
 & Baseline & Ours &  {\sc model\_inv} & Baseline & Ours & {\sc model\_inv} \\ \hline
Inconsistently labeled & \textbf{66.3 $\pm$ 1.8} & 65.2 $\pm$ 1.9 & 65.0 $\pm$ 1.8 & 19.6 $\pm$ 4.3 & \textbf{14.5 $\pm$ 4.1} & 20.4 $\pm$ 4.2 \\
Gender-dependent & \textbf{78.6 $\pm$ 1.4} & 77.8 $\pm$ 1.4 & 77.5 $\pm$ 1.4 & 23.0 $\pm$ 3.6 & \textbf{21.8 $\pm$ 3.8} & 25.6 $\pm$ 3.4 \\
Gender-independent & \textbf{83.9 $\pm$ 1.5} & 83.0 $\pm$ 1.6 & 83.3 $\pm$ 1.6 & 16.6 $\pm$ 5.1 & \textbf{13.6 $\pm$ 5.1} & 16.0 $\pm$ 5.0 \\ \hline

 & \multicolumn{3}{c}{DNAP $\downarrow$} & \multicolumn{3}{|c|}{Bias Amplification $\downarrow$} \\ \hline
Inconsistently labeled & 10.2 $\pm$ 3.7 & 9.9 $\pm$ 3.6 & \textbf{9.1 $\pm$ 3.3} & 2.6 $\pm$ 0.2 & 1.8 $\pm$ 0.2 & \textbf{1.5 $\pm$ 0.2} \\
Gender-dependent & \textbf{7.6 $\pm$ 2.3} & 7.8 $\pm$ 2.7 & \textbf{7.6 $\pm$ 2.3} & 2.2 $\pm$ 0.2 & \textbf{1.7 $\pm$ 0.2} & 2.1 $\pm$ 0.2 \\
Gender-independent & 3.6 $\pm$ 3.0 & 3.6 $\pm$ 3.2 & \textbf{3.2 $\pm$ 2.8} & 1.0 $\pm$ 0.2 & \textbf{0.6 $\pm$ 0.2} & 0.8 $\pm$ 0.2 \\ \hline
\end{tabular}

% Attribute-level table
%\begin{comment}
\begin{tabular}{l|ccc|ccc|ccc|ccc|}
\cline{2-13}
 & \multicolumn{3}{c|}{AP $\uparrow$} & \multicolumn{3}{c|}{Difference in Equality of Opportunity $\downarrow$} & \multicolumn{3}{c|}{Difference in Normalized AP $\downarrow$} & \multicolumn{3}{c|}{Bias Amplification $\downarrow$} \\ \cline{2-13} 
 & \multicolumn{1}{c}{Baseline} & Ours & {\sc model\_inv} & \multicolumn{1}{c}{Baseline} & Ours & {\sc model\_inv} & \multicolumn{1}{c}{Baseline} & Ours & {\sc model\_inv} & \multicolumn{1}{c}{Baseline} & Ours & {\sc model\_inv} \\ \hline
\multicolumn{13}{|l|}{\textbf{Type 1 Attributes}} \\ \hline
\multicolumn{1}{|l|}{\tt BigLips} & \textbf{58.9 $\pm$ 1.2} & 58.7 $\pm$ 1.2 & 57.0 $\pm$ 1.3 & {4.4 $\pm$ 2.7} & \textbf{1.1 $\pm$ 1.9} & 1.3 $\pm$ 2.0 & 25.2 $\pm$ 2.2 & 25.7 $\pm$ 2.3 & \textbf{25.1 $\pm$ 2.1} & 4.5 $\pm$ 0.3 & 4.4 $\pm$ 0.2 & \textbf{1.9 $\pm$ 0.2} \\
\multicolumn{1}{|l|}{\tt BigNose} & \textbf{68.6 $\pm$ 1.4} & 68.0 $\pm$ 1.4 & 67.2 $\pm$ 1.4 & 32.3 $\pm$ 3.1 & \textbf{20.1 $\pm$ 2.9} & {36.4 $\pm$ 3.1} & 14.8 $\pm$ 2.8 & \textbf{13.8 $\pm$ 2.8} & 16.8 $\pm$ 2.8 & 4.6 $\pm$ 0.3 & \textbf{2.6 $\pm$ 0.3} & 3.9 $\pm$ 0.3 \\
\multicolumn{1}{|l|}{\tt OvalFace} & \textbf{57.6 $\pm$ 1.3} & 55.8 $\pm$ 1.3 & 52.8 $\pm$ 1.4 & {25.9 $\pm$ 2.7} & 19.7 $\pm$ 2.7 & \textbf{18.6 $\pm$ 2.7} & 4.3 $\pm$ 2.6 & 4.2 $\pm$ 2.5 & \textbf{0.8 $\pm$ 1.6} & 3.6 $\pm$ 0.4 & 1.5 $\pm$ 0.4 & \textbf{0.3 $\pm$ 0.1} \\
\multicolumn{1}{|l|}{\tt PaleSkin} & \textbf{67.7 $\pm$ 3.4} & 65.8 $\pm$ 3.5 & 67.4 $\pm$ 3.4 & 17.2 $\pm$ 8.4 & 15.3 $\pm$ 8.3 & \textbf{12.7 $\pm$ 8.3} & 10.2 $\pm$ 7.1 & 7.7 $\pm$ 6.8 & \textbf{5.6 $\pm$ 6.5} & \textbf{0.2 $\pm$ 0.1} & \textbf{0.2 $\pm$ 0.1} & \textbf{0.2 $\pm$ 0.1} \\
\multicolumn{1}{|l|}{\tt StraightHair} & 59.2 $\pm$ 1.6 & 57.5 $\pm$ 1.7 & \textbf{59.4 $\pm$ 1.6} & 1.9 $\pm$ 2.6 & \textbf{1.8 $\pm$ 2.5} & {7.2 $\pm$ 3.0} & 4.7 $\pm$ 2.9 & 5.6 $\pm$ 3.0 & \textbf{1.9 $\pm$ 2.5} & 0.6 $\pm$ 0.2 & 1.0 $\pm$ 0.3 & \textbf{0.3 $\pm$ 0.2} \\
\multicolumn{1}{|l|}{\tt WavyHair} & 85.8 $\pm$ 0.7 & 85.2 $\pm$ 0.7 & \textbf{86.4 $\pm$ 0.7} & 35.8 $\pm$ 3.1 & \textbf{29.1 $\pm$ 3.2} & 45.9 $\pm$ 2.9 & \textbf{1.8 $\pm$ 1.7} & 2.6 $\pm$ 1.9 & 4.5 $\pm$ 1.9 & 1.8 $\pm$ 0.3 & \textbf{1.3 $\pm$ 0.2} & 2.3 $\pm$ 0.3 \\ \hline
\multicolumn{1}{|l|}{\textbf{Average}} & \textbf{66.3 $\pm$ 1.8} & 65.2 $\pm$ 1.9 & 65.0 $\pm$ 1.8 & 19.6 $\pm$ 4.3 & \textbf{14.5 $\pm$ 4.1} & 20.4 $\pm$ 4.2 & 10.2 $\pm$ 3.7 & 9.9 $\pm$ 3.6 & \textbf{9.1 $\pm$ 3.3} & 2.6 $\pm$ 0.2 & 1.8 $\pm$ 0.2 & \textbf{1.5 $\pm$ 0.2} \\ \hline
\multicolumn{13}{|l|}{\textbf{Type 2 Attributes}} \\ \hline
\multicolumn{1}{|l|}{\tt ArchedBrows} & \textbf{78.5 $\pm$ 1.0} & 77.9 $\pm$ 1.1 & 77.7 $\pm$ 1.1 & \textbf{36.1 $\pm$ 4.7} & {40.0 $\pm$ 5.0} & 47.2 $\pm$ 4.5 & 13.1 $\pm$ 2.5 & 12.8 $\pm$ 2.8 & \textbf{11.2 $\pm$ 2.7} & 4.8 $\pm$ 0.3 & \textbf{4.3 $\pm$ 0.2} & 4.6 $\pm$ 0.3 \\ 
\multicolumn{1}{|l|}{\tt Attractive} & \textbf{91.4 $\pm$ 0.5} & 91.0 $\pm$ 0.4 & 90.6 $\pm$ 0.5 & \textbf{16.5 $\pm$ 1.9} & 18.4 $\pm$ 2.0 & 16.7 $\pm$ 2.3 & 4.3 $\pm$ 1.2 & \textbf{3.9 $\pm$ 1.2} & 4.6 $\pm$ 1.3 & 1.8 $\pm$ 0.3 & \textbf{1.4 $\pm$ 0.3} & \textbf{0.6 $\pm$ 0.2} \\
\multicolumn{1}{|l|}{\tt BushyBrows} & \textbf{79.2 $\pm$ 1.4} & 78.0 $\pm$ 1.5 & 77.0 $\pm$ 1.5 & 32.0 $\pm$ 4.2 & \textbf{23.0 $\pm$ 4.0} & {33.9 $\pm$ 3.8} & \textbf{18.1 $\pm$ 3.1} & 20.1 $\pm$ 3.4 & 19.8 $\pm$ 3.6 & 0.8 $\pm$ 0.2 & \textbf{0.2 $\pm$ 0.1} & 1.1 $\pm$ 0.2 \\
\multicolumn{1}{|l|}{\tt PointyNose} & \textbf{64.1 $\pm$ 1.3} & 62.8 $\pm$ 1.3 & 63.2 $\pm$ 1.4 & 31.5 $\pm$ 3.1 & \textbf{30.2 $\pm$ 3.2} & {31.9 $\pm$ 3.0} & 7.2 $\pm$ 2.6 & \textbf{7.0 $\pm$ 2.5} & 7.3 $\pm$ 2.6 & \textbf{2.9 $\pm$ 0.3} & \textbf{2.9 $\pm$ 0.2} & 3.9 $\pm$ 0.3 \\
\multicolumn{1}{|l|}{\tt RecedingHair} & \textbf{61.6 $\pm$ 2.5} & 60.2 $\pm$ 2.5 & 59.8 $\pm$ 2.6 & {16.8 $\pm$ 5.0} & \textbf{13.7 $\pm$ 4.7} & 17.7 $\pm$ 4.5 & \textbf{1.7 $\pm$ 2.6} & 2.0 $\pm$ 3.5 & 1.8 $\pm$ 3.3 & 1.3 $\pm$ 0.2 & \textbf{0.7 $\pm$ 0.1} & 1.1 $\pm$ 0.2 \\
\multicolumn{1}{|l|}{\tt Young} & \textbf{97.0 $\pm$ 0.3} & 96.8 $\pm$ 0.3 & 96.9 $\pm$ 0.3 & \textbf{5.2 $\pm$ 0.8} & \textbf{5.2 $\pm$ 0.8} & 6.4 $\pm$ 0.9 & 1.1 $\pm$ 0.6 & \textbf{1.0 $\pm$ 0.5} & 1.1 $\pm$ 0.5 & 1.4 $\pm$ 0.3 & \textbf{0.9 $\pm$ 0.3} & 1.6 $\pm$ 0.2 \\ \hline
\multicolumn{1}{|l|}{\textbf{Average}} & \textbf{78.6 $\pm$ 1.4} & 77.8 $\pm$ 1.4 & 77.5 $\pm$ 1.4 & 23.0 $\pm$ 3.6 & \textbf{21.8 $\pm$ 3.8} & 25.6 $\pm$ 3.4 & \textbf{7.6 $\pm$ 2.3} & 7.8 $\pm$ 2.7 & \textbf{7.6 $\pm$ 2.3} & 2.2 $\pm$ 0.2 & \textbf{1.7 $\pm$ 0.2} & 2.1 $\pm$ 0.2 \\ \hline
\multicolumn{13}{|l|}{\textbf{Type 3 Attributes}} \\ \hline
\multicolumn{1}{|l|}{\tt Bangs} & \textbf{94.9 $\pm$ 0.6} & 94.4 $\pm$ 0.6 & 94.4 $\pm$ 0.6 & {4.6 $\pm$ 3.4} & 3.6 $\pm$ 3.3 & \textbf{3.3 $\pm$ 3.5} & 2.7 $\pm$ 1.1 & \textbf{2.6 $\pm$ 1.1} & 3.1 $\pm$ 1.3 & 0.4 $\pm$ 0.1 & \textbf{0.3 $\pm$ 0.1} & \textbf{0.3 $\pm$ 0.1} \\
\multicolumn{1}{|l|}{\tt BlackHair} & \textbf{88.4 $\pm$ 0.8} & 87.4 $\pm$ 0.8 & 88.3 $\pm$ 0.8 & 3.1 $\pm$ 2.3 & {0.9 $\pm$ 1.7} & \textbf{0.8 $\pm$ 1.5} & 4.2 $\pm$ 1.5 & 5.0 $\pm$ 1.6 & \textbf{3.7 $\pm$ 1.5} & 0.6 $\pm$ 0.2 & \textbf{0.3 $\pm$ 0.1} & 0.5 $\pm$ 0.2 \\
\multicolumn{1}{|l|}{\tt BlondHair} & 91.3 $\pm$ 0.9 & 90.5 $\pm$ 1.0 & \textbf{91.5 $\pm$ 0.9} & \textbf{44.0 $\pm$ 7.7} & 44.2 $\pm$ 7.9 & {45.8 $\pm$ 7.4} & 3.8 $\pm$ 3.7 & 4.1 $\pm$ 3.9 & \textbf{3.5 $\pm$ 3.5} & 1.4 $\pm$ 0.1 & 0.8 $\pm$ 0.1 & \textbf{0.6 $\pm$ 0.1} \\
\multicolumn{1}{|l|}{\tt BrownHair} & \textbf{74.1 $\pm$ 1.4} & 73.5 $\pm$ 1.4 & 74.0 $\pm$ 1.5 & \textbf{4.0 $\pm$ 2.9} & {5.3 $\pm$ 3.0} & 8.0 $\pm$ 3.1 & 4.9 $\pm$ 2.7 & \textbf{2.8 $\pm$ 2.9} & 6.6 $\pm$ 2.9 & 0.8 $\pm$ 0.2 & \textbf{0.7 $\pm$ 0.2} & 1.6 $\pm$ 0.3 \\
\multicolumn{1}{|l|}{\tt Chubby} & \textbf{58.1 $\pm$ 3.2} & 56.3 $\pm$ 3.1 & 54.1 $\pm$ 3.3 & 30.7 $\pm$ 8.7 & \textbf{26.1 $\pm$ 8.9} & {35.9 $\pm$ 8.3} & 4.7 $\pm$ 6.1 & 4.3 $\pm$ 6.3 & \textbf{2.7 $\pm$ 5.0} & 2.0 $\pm$ 0.1 & \textbf{0.5 $\pm$ 0.1} & 0.8 $\pm$ 0.1 \\
\multicolumn{1}{|l|}{\tt Earrings} & \textbf{82.8 $\pm$ 1.1} & 82.1 $\pm$ 1.1 & 82.7 $\pm$ 1.0 & 49.4 $\pm$ 7.2 & \textbf{41.0 $\pm$ 7.3} & 49.3 $\pm$ 7.0 & 5.2 $\pm$ 3.9 & 7.8 $\pm$ 3.4 & \textbf{2.2 $\pm$ 3.2} & 2.7 $\pm$ 0.1 & 3.0 $\pm$ 0.2 & \textbf{1.7 $\pm$ 0.1} \\ 
\multicolumn{1}{|l|}{\tt EyeBags} & \textbf{65.4 $\pm$ 1.7} & 63.7 $\pm$ 1.7 & 64.3 $\pm$ 1.7 & 24.3 $\pm$ 3.2 & {16.4 $\pm$ 3.2} & \textbf{15.4 $\pm$ 2.9} & \textbf{1.3 $\pm$ 2.2} & 1.4 $\pm$ 2.3 & 1.4 $\pm$ 2.5 & 3.6 $\pm$ 0.2 & \textbf{2.2 $\pm$ 0.3} & 3.8 $\pm$ 0.3 \\
\multicolumn{1}{|l|}{\tt Glasses} & \textbf{99.1 $\pm$ 0.5} & 98.8 $\pm$ 0.5 & 98.7 $\pm$ 0.5 & {1.0 $\pm$ 1.7} & {1.0 $\pm$ 1.6} & \textbf{0.7 $\pm$ 1.4} & 1.0 $\pm$ 1.0 & \textbf{0.8 $\pm$ 1.0} & \textbf{0.8 $\pm$ 0.9} & 0.3 $\pm$ 0.1 & \textbf{0.0 $\pm$ 0.1} & \textbf{0.1 $\pm$ 0.1} \\
\multicolumn{1}{|l|}{\tt GrayHair} & 77.1 $\pm$ 3.2 & 74.7 $\pm$ 3.5 & \textbf{77.3 $\pm$ 3.2} & 32.4 $\pm$ 9.8 & \textbf{20.5 $\pm$ 10.1} & {27.2 $\pm$ 9.8} & 3.2 $\pm$ 5.2 & 4.8 $\pm$ 6.1 & \textbf{2.8 $\pm$ 4.7} & 1.3 $\pm$ 0.1 & \textbf{0.8 $\pm$ 0.1} & 1.0 $\pm$ 0.2 \\
\multicolumn{1}{|l|}{\tt HighCheeks} & \textbf{95.4 $\pm$ 0.3} & 95.1 $\pm$ 0.3 & 95.1 $\pm$ 0.3 & \textbf{11.8 $\pm$ 1.9} & 13.6 $\pm$ 1.9 & 14.5 $\pm$ 2.0 & \textbf{4.4 $\pm$ 0.7} & 4.8 $\pm$ 0.8 & 4.9 $\pm$ 0.8 & \textbf{0.1 $\pm$ 0.2} & \textbf{0.1 $\pm$ 0.1} & 0.2 $\pm$ 0.2 \\
\multicolumn{1}{|l|}{\tt MouthOpen} & \textbf{98.8 $\pm$ 0.1} & 98.7 $\pm$ 0.1 & 98.6 $\pm$ 0.1 & {1.5 $\pm$ 1.0} & 1.1 $\pm$ 1.2 & \textbf{0.7 $\pm$ 1.0} & 0.3 $\pm$ 0.2 & \textbf{0.2 $\pm$ 0.2} & \textbf{0.2 $\pm$ 0.2} & 0.1 $\pm$ 0.1 & 0.1 $\pm$ 0.1 & \textbf{0.0 $\pm$ 0.0} \\
\multicolumn{1}{|l|}{\tt NarrowEyes} & \textbf{56.3 $\pm$ 1.9} & 55.3 $\pm$ 2.0 & 53.8 $\pm$ 2.0 & 15.6 $\pm$ 3.8 & \textbf{10.6 $\pm$ 3.5} & {14.5 $\pm$ 3.7} & 11.8 $\pm$ 3.3 & \textbf{10.3 $\pm$ 3.7} & 11.1 $\pm$ 3.6 & \textbf{0.0 $\pm$ 0.4} & 0.1 $\pm$ 0.2 & \textbf{0.0 $\pm$ 0.4} \\
\multicolumn{1}{|l|}{\tt Smiling} & \textbf{98.4 $\pm$ 0.1} & 98.3 $\pm$ 0.1 & 98.3 $\pm$ 0.1 & {4.7 $\pm$ 1.2} & \textbf{3.0 $\pm$ 1.2} & {4.0 $\pm$ 1.3} & \textbf{0.5 $\pm$ 0.3} & \textbf{0.5 $\pm$ 0.3} & \textbf{0.5 $\pm$ 0.3} & 0.3 $\pm$ 0.2 & \textbf{0.0 $\pm$ 0.1} & \textbf{0.0 $\pm$ 0.1} \\
\multicolumn{1}{|l|}{\tt WearingHat} & 94.7 $\pm$ 1.1 & 93.8 $\pm$ 1.3 & \textbf{94.8 $\pm$ 1.3} & {4.8 $\pm$ 4.8} & \textbf{3.1 $\pm$ 4.0} & {3.2 $\pm$ 4.2} & 2.2 $\pm$ 2.5 & \textbf{1.1 $\pm$ 1.8} & 1.8 $\pm$ 2.3 & 0.2 $\pm$ 0.1 & \textbf{0.1 $\pm$ 0.1} & \textbf{0.1 $\pm$ 0.1} \\ \hline
\multicolumn{1}{|l|}{\textbf{Average}} & \textbf{83.9 $\pm$ 1.5} & 83.0 $\pm$ 1.6 & 83.3 $\pm$ 1.6 & 16.6 $\pm$ 5.1 & \textbf{13.6 $\pm$ 5.1} & 16.0 $\pm$ 5.0 & 3.6 $\pm$ 3.0 & 3.6 $\pm$ 3.2 & \textbf{3.2 $\pm$ 2.8} & 1.0 $\pm$ 0.2 & \textbf{0.6 $\pm$ 0.2} & 0.8 $\pm$ 0.2 \\ \hline
\end{tabular}
\end{comment}


\begin{comment}
\begin{tabular}{|c|c|c||c|c||c|c|}
\hline
\multirow{3}{*}{\textbf{Attribute}} & \multicolumn{2}{c||}{\multirow{2}{*}{\textbf{Average Precision}}} & \multicolumn{2}{c||}{\textbf{Diff. in equality}} & \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Bias amplification}}} \\  
& \multicolumn{2}{c||}{} &\multicolumn{2}{c||}{\textbf{of opportunity}} & \multicolumn{2}{c|}{}\\\cline{2-7}
 & \textbf{Baseline}  & \textbf{Model} & \textbf{Baseline} & \textbf{Model} & \textbf{Baseline} & \textbf{Model} \\ \hline
\texttt{ArchedEyebrows} & 78.6 $\pm$ 1.1 & 78.1 $\pm$ 1.1 & 5.55 & \textbf{4.26} & \textbf{0.023} & 0.026 \\
\texttt{Attractive} & 91.4 $\pm$ 0.4 & 91.1 $\pm$ 0.5 & \textbf{2.47} & 2.71 & \textbf{None} & \textbf{None} \\
\texttt{BagsUnderEyes} & 65.4 $\pm$ 1.7 & 63.6 $\pm$ 1.7 & 3.67 & \textbf{2.35} & 0.058 & \textbf{0.052} \\
\texttt{Bangs} & 94.9 $\pm$ 0.5 & 94.8 $\pm$ 0.5 & \textbf{1.55} & 1.58 & \textbf{None} & \textbf{None} \\
\texttt{BigLips} & 59.0 $\pm$ 1.2 & 57.8 $\pm$ 1.2 & 9.51 & \textbf{8.78} & \textbf{0.074} & 0.078 \\
\texttt{BigNose} & 68.6 $\pm$ 1.4 & 68.4 $\pm$ 1.4 & \textbf{1.64} & 1.79 & 0.053 & \textbf{0.040} \\
\texttt{BlackHair} & 88.4 $\pm$ 0.8 & 87.8 $\pm$ 0.8 & \textbf{1.19} & 1.25 & \textbf{None} & \textbf{None} \\
\texttt{BlondHair} & 91.3 $\pm$ 0.9 & 90.9 $\pm$ 1.0 & 0.81 & \textbf{0.62} & 0.022 & \textbf{0.008} \\
\texttt{BrownHair} & 74.0 $\pm$ 1.4 & 73.6 $\pm$ 1.5 & 0.94 & \textbf{0.20} & \textbf{None} & \textbf{None} \\
\texttt{BushyEyebrows} & 79.2 $\pm$ 1.4 & 78.0 $\pm$ 1.4 & 0.82 & \textbf{0.69} & \textbf{0.043} & 0.066 \\
\texttt{Chubby} & 58.0 $\pm$ 3.2 & 57.2 $\pm$ 3.4 & 2.78 & \textbf{2.66} & \textbf{0.031} & 0.038 \\
\texttt{Eyeglasses} & 99.1 $\pm$ 0.5 & 98.8 $\pm$ 0.5 & 0.28 & \textbf{0.24} & 0.003 & \textbf{0.002} \\
\texttt{GrayHair} & 77.1 $\pm$ 3.1 & 76.0 $\pm$ 3.2 & \textbf{0.80} & 0.96 & 0.047 & \textbf{0.026} \\
\texttt{HighCheekbones} & 95.4 $\pm$ 0.3 & 95.2 $\pm$ 0.3 & \textbf{0.53} & 1.69 & \textbf{None} & 0.003 \\
\texttt{MouthSlightlyOpen} & 98.8 $\pm$ 0.1 & 98.7 $\pm$ 0.1 & \textbf{0.02} & 0.15 & \textbf{None} & \textbf{None} \\
\texttt{NarrowEyes} & 56.3 $\pm$ 2.0 & 55.7 $\pm$ 2.0 & 2.96 & \textbf{2.62} & \textbf{None} & \textbf{None} \\
\texttt{OvalFace} & 57.5 $\pm$ 1.4 & 56.2 $\pm$ 1.3 & 4.18 & \textbf{3.32} & 0.048 & \textbf{0.017} \\
\texttt{PaleSkin} & 67.8 $\pm$ 3.6 & 66.6 $\pm$ 3.6 & \textbf{0.54} & 0.65 & 0.023 & \textbf{0.004} \\
\texttt{PointyNose} & 64.1 $\pm$ 1.3 & 63.7 $\pm$ 1.4 & 0.19 & \textbf{0.15} & 0.063 & \textbf{0.037} \\
\texttt{RecedingHairline} & 61.7 $\pm$ 2.5 & 59.4 $\pm$ 2.6 & 0.99 & \textbf{0.76} & \textbf{0.074} & 0.099 \\
\texttt{Smiling} & 98.4 $\pm$ 0.1 & 98.4 $\pm$ 0.1 & 0.79 & \textbf{0.09} & 0.003 & \textbf{None} \\
\texttt{StraightHair} & 59.1 $\pm$ 1.6 & 57.1 $\pm$ 1.7 & 2.52 & \textbf{0.79} & 0.001 & \textbf{None} \\
\texttt{WavyHair} & 85.8 $\pm$ 0.7 & 85.2 $\pm$ 0.7 & \textbf{2.91} & 4.81 & \textbf{0.056} & 0.069 \\
\texttt{WearingEarrings} & 82.8 $\pm$ 1.1 & 82.0 $\pm$ 1.1 & \textbf{4.12} & 5.73 & \textbf{0.018} & 0.020 \\
\texttt{WearingHat} & 94.8 $\pm$ 1.1 & 94.2 $\pm$ 1.2 & 0.36 & \textbf{0.33} & \textbf{None} & \textbf{None} \\
\texttt{Young} & 97.0 $\pm$ 0.2 & 97.0 $\pm$ 0.2 & \textbf{2.80} & 3.24 & \textbf{None} & \textbf{None} \\ \hline
\textbf{Average} & 78.6 $\pm$ 1.6 & 77.9 $\pm$ 1.6 & 2.08 & \textbf{1.97} & 0.025 & \textbf{0.022} \\ \hline
\end{tabular}
\end{comment}


==> GAN debiasing CVPR/full_skew_results.tex <==
    \begin{tabular}{c | c c c c c c c c c c c c c c c c c c c c c c c c c c}

    & \rot{\texttt{ArchedBrows}} 
    & \rot{\texttt{Attractive}}
    & \rot{\texttt{Bangs}}
    %& \rot{\texttt{BigLips}}
    %& \rot{\texttt{BigNose}}
    & \rot{\texttt{BlackHair}}
    & \rot{\texttt{BlondHair}}
    & \rot{\texttt{BrownHair}}
    & \rot{\texttt{BushyBrows}}
    & \rot{\texttt{Chubby}}
    & \rot{\texttt{Earrings}}
    & \rot{\texttt{EyeBags}}
    & \rot{\texttt{Glasses}}
    & \rot{\texttt{GrayHair}}
    & \rot{\texttt{HighCheeks}}
    & \rot{\texttt{MouthOpen}}
    & \rot{\texttt{NarrowEyes}}
    %& \rot{\texttt{OvalFace}}
    %& \rot{\texttt{PaleSkin}}
    & \rot{\texttt{PointyNose}}
    & \rot{\texttt{RecedingHair}}
    & \rot{\texttt{Smiling}}
    %& \rot{\texttt{StraightHair}}
    %& \rot{\texttt{WavyHair}}
    & \rot{\texttt{WearingHat}}
    & \rot{\texttt{Young}} \\
    \hline
    \texttt{Gender} & \texttt{y} & \texttt{y} & \texttt{y} & % \texttt{y} & \texttt{y} & 
    \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & \texttt{n} & \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & %\texttt{y} & \texttt{y} &
    \texttt{y} & \texttt{y} & \texttt{y} & % \texttt{y} & \texttt{y} & 
   \texttt{n} & \texttt{y} \\
    \texttt{Glasses} & \texttt{y} & \texttt{y} & \texttt{y} & % \texttt{y} & \texttt{y} & 
    \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & -- & \texttt{y} & \texttt{y} & \texttt{y} & \texttt{y} & %\texttt{y} & \texttt{y} & 
    \texttt{y} & \texttt{y} & \texttt{y} & %\texttt{y} & \texttt{y} & 
    \texttt{y} & \texttt{y} \\
    \texttt{Young} & \texttt{n} & \texttt{n} &  \texttt{n} & %\texttt{y} & \texttt{y} & 
    \texttt{n} & \texttt{n} & \texttt{y} & \texttt{n} & \texttt{n} & \texttt{y} & \texttt{n} & \texttt{n} & \texttt{n} & \texttt{n} & \texttt{n} & \texttt{n} & %\texttt{y} & \texttt{n} &
    \texttt{y} & \texttt{n} & \texttt{n} & %\texttt{y} & \texttt{y} & 
     \texttt{y} & -- \\
    \hline
    \end{tabular}


==> GAN debiasing CVPR/gender_exp_manipulation.tex <==
\begin{tabular}{c c c c c c}
\multicolumn{6}{c}{\texttt{Eyeglasses}} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_0.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_49.jpg} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_10.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_49.jpg} \\
\multicolumn{6}{c}{\texttt{BlondHair}} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_0.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_49.jpg} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_10.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_49.jpg} \\
\multicolumn{6}{c}{\texttt{Smiling}} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_0.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_49.jpg} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_10.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_49.jpg} \\

\end{tabular}

==> gender_exp_manipulation.tex <==
\begin{tabular}{c c c c c c}
\multicolumn{6}{c}{\texttt{Eyeglasses}} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_0.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_no_perp/gen_49.jpg} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_10.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Glasses_perp/gen_49.jpg} \\
\multicolumn{6}{c}{\texttt{BlondHair}} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_0.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_no_perp/gen_49.jpg} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_10.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Blond_perp/gen_49.jpg} \\
\multicolumn{6}{c}{\texttt{Smiling}} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_0.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_no_perp/gen_49.jpg} \\
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_0.jpg} & 
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_10.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_20.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_30.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_40.jpg} &
\includegraphics[width=0.12\textwidth]{ImagesAppendix/Smiling_perp/gen_49.jpg} \\

\end{tabular}
